When and why vision-language models behave like bags-of-words, and what to do about it?

Despite the success of large vision and language models (VLMs) in many downstream applications, it is unclear how well they encode compositional information. Here, we create the Attribution, Relation, and Order (ARO) benchmark to systematically evaluate the ability of VLMs to understand different types of relationships, attributes, and order. ARO consists of Visual Genome Attribution, to test the understanding of objects' properties; Visual Genome Relation, to test for relational understanding; and COCO & Flickr30k-Order, to test for order sensitivity. ARO is orders of magnitude larger than previous benchmarks of compositionality, with more than 50,000 test cases. We show where state-of-the-art VLMs have poor relational understanding, can blunder when linking objects to their attributes, and demonstrate a severe lack of order sensitivity. VLMs are predominantly trained and evaluated on large datasets with rich compositional structure in the images and captions. Yet, training on these datasets has not been enough to address the lack of compositional understanding, and evaluating on these datasets has failed to surface this deficiency. To understand why these limitations emerge and are not represented in the standard tests, we zoom into the evaluation and training procedures. We demonstrate that it is possible to perform well on retrieval over existing datasets without using the composition and order information. Given that contrastive pretraining optimizes for retrieval on datasets with similar shortcuts, we hypothesize that this can explain why the models do not need to learn to represent compositional information. This finding suggests a natural solution: composition-aware hard negative mining. We show that a simple-to-implement modification of contrastive learning significantly improves the performance on tasks requiring understanding of order and compositionality.

==> trash.tex <==
\begin{table}[!th]
    \centering
    \caption{COCO Zero-shot Retrieval Experiments}

\begin{tabular}{lllll}
\toprule
\textbf{COCO Zero-shot Retrieval} \\
Text Perturbation Strategy &       ImagePrec@1 &        TextPrec@1 &       ImagePrec@5 &        TextPrec@5 \\
\toprule
\midrule
Shuffle Else                &  $26.33 \pm 0.29$ &  $41.23 \pm 0.43$ &  $50.91 \pm 0.40$ &  $67.17 \pm 0.41$ \\
Shuffle Nouns And Adj       &  $25.64 \pm 0.39$ &  $41.70 \pm 0.36$ &  $50.24 \pm 0.43$ &  $67.67 \pm 0.33$ \\
Shuffle Trigrams            &  $26.24 \pm 0.42$ &  $41.40 \pm 0.45$ &  $51.53 \pm 0.29$ &  $67.42 \pm 0.38$ \\
Shuffle Within Trigrams     &  $25.57 \pm 0.32$ &  $40.35 \pm 0.47$ &  $50.13 \pm 0.39$ &  $66.39 \pm 0.35$ \\
Shuffle Words               &  $21.83 \pm 0.31$ &  $34.34 \pm 0.30$ &  $44.34 \pm 0.59$ &  $60.80 \pm 0.50$ \\
\midrule
No Perturbations                &   $31.66$ &   $50.12$ &   $58.24$ &   $74.80$ \\
\bottomrule
\toprule

\textbf{Flickr30k Zero-shot Retrieval}               \\
Text Perturbation Strategy &       ImagePrec@1 &        TextPrec@1 &       ImagePrec@5 &        TextPrec@5 \\
\toprule
\midrule
Shuffle Else                &  $52.45 \pm 0.64$ &  $67.71 \pm 0.98$ &  $79.43 \pm 0.87$ &  $90.32 \pm 0.56$ \\

Shuffle Nouns And Adj       &  $52.18 \pm 1.01$ &  $68.99 \pm 1.36$ &  $78.79 \pm 0.45$ &  $91.10 \pm 0.94$ \\
Shuffle Trigrams            &  $52.62 \pm 0.78$ &  $68.88 \pm 0.87$ &  $79.58 \pm 0.71$ &  $91.42 \pm 0.72$ \\
Shuffle Within Trigrams     &  $54.05 \pm 1.32$ &  $69.69 \pm 1.00$ &  $80.35 \pm 0.55$ &  $91.19 \pm 0.61$ \\
Shuffle Words               &  $44.18 \pm 0.78$ &  $57.42 \pm 1.17$ &  $71.47 \pm 0.79$ &  $83.98 \pm 1.08$ \\
\midrule
No Perturbations                &   $61.40$ &   $80.60$ &   $85.50$ &   $96.00$ \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!th]
    \centering
    \caption{COCO Zero-shot Retrieval Experiments}

\begin{tabular}{lllll}
\toprule
\textbf{COCO Zero-shot Retrieval}               \\
Image Perturbation Strategy &       ImagePrec@1 &        TextPrec@1 &       ImagePrec@5 &        TextPrec@5 \\
\midrule
Shuffle All Patches           &  $18.67 \pm 0.45$ &  $20.96 \pm 0.45$ &  $39.64 \pm 0.23$ &  $43.56 \pm 0.38$ \\
Shuffle Rows               &  $23.86 \pm 0.49$ &  $35.74 \pm 0.48$ &  $47.87 \pm 0.70$ &  $60.34 \pm 0.57$ \\
Shuffle Columns               &  $26.16 \pm 0.61$ &  $38.90 \pm 0.37$ &  $50.37 \pm 0.56$ &  $63.74 \pm 0.34$ \\

\midrule
No Perturbations&   $31.66$ &   $50.12 $ &   $58.24$ &   $74.80$ \\
\bottomrule
\toprule

\textbf{Flickr30k Zero-shot Retrieval}               \\
Image Perturbation Strategy &       ImagePrec@1 &        TextPrec@1 &       ImagePrec@5 &        TextPrec@5 \\
\toprule
\midrule
Shuffle All Patches            &  $36.69 \pm 1.89$ &  $46.68 \pm 1.33$ &  $62.95 \pm 1.92$ &  $72.74 \pm 1.29$ \\
Shuffle Rows               &  $46.88 \pm 1.44$ &  $59.64 \pm 0.70$ &  $72.82 \pm 1.23$ &  $83.59 \pm 0.93$ \\
Shuffle Columns               &  $49.92 \pm 1.59$ &  $66.87 \pm 0.82$ &  $77.61 \pm 0.98$ &  $88.63 \pm 0.37$ \\
\midrule
No Perturbations                &   $61.40$ &   $80.60$ &   $85.50$ &   $96.00$ \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!th]
    \centering
    \caption{Winoground and Visual-Genome Relation Tests}
\begin{tabular}{llll | l}
\toprule
& \textbf{Winoground}         & &  & \textbf{Visual Genome Relations}    \\

Image Perturbation Strategy & Image & Text & Group & Accuracy \\
\midrule
Shuffle Columns               &  $11.25 \pm 1.15$ &  $29.33 \pm 1.32$ &  $8.43 \pm 0.81$ &  $45.14 \pm 0.10$ \\
Shuffle Patches            &   $9.38 \pm 0.84$ &  $27.22 \pm 1.54$ &  $6.58 \pm 0.82$ &  $45.12 \pm 0.24$ \\
Shuffle Rows               &   $9.47 \pm 1.20$ &  $28.02 \pm 1.52$ &  $6.28 \pm 0.83$  &  $45.40 \pm 0.21$ \\
\midrule
No Perturbation    &   $10.50$ &   $31.00 $ &   $8.50 $ & $46.85$ \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[!th]
    \centering
    \caption{Winoground Text Perturbations}
\begin{tabular}{llll}
\toprule
\textbf{Winoground} \\
Text Perturbation Strategy &             Image &              Text &            Group \\
\midrule
Shuffle Else                &   $9.35 \pm 1.08$ &  $20.40 \pm 1.92$ &  $5.65 \pm 1.24$ \\
Shuffle Nouns And Adj       &   $7.10 \pm 1.09$ &  $16.80 \pm 1.99$ &  $4.30 \pm 0.86$ \\
Shuffle Within Trigrams     &   $8.88 \pm 1.09$ &  $16.35 \pm 1.55$ &  $4.05 \pm 0.75$ \\
Shuffle Words               &   $7.92 \pm 1.39$ &  $14.45 \pm 1.27$ &  $3.65 \pm 1.19$ \\
Shuffle Trigrams            &  $11.05 \pm 1.54$ &  $21.75 \pm 1.44$ &  $6.18 \pm 1.09$ \\
\midrule
Shuffle None                &   $10.50$ &   $31.00 $ &   $8.50 $ \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}[t]
\centering
\caption{\textbf{Large-scale benchmarks to test relational and attributive understanding.}  Here, we propose two large scale datasets to test the model's ability to identify relations and property attribution. Concretely, we probe the models' ability to pick the correct ordering of the constituents of a relation, e.g. by asking the model to pick between `the horse is eating the grass' vs `the grass is eating the horse' (see the top figure). Existing VLMs exhibit intriguing inabilities at this simple task, where several models remain at, or below the chance-level (50\%).
}
\label{appendix:fig:winoground-relations}
\includegraphics[clip, trim=0cm 5cm 0cm 0cm, width=\textwidth]{figures/winoground_relations.pdf}
\end{figure}


